Jaccard-constrained dense subgraph discovery

Finding dense subgraphs is a core problem in graph mining with many applications in diverse domains. At the same time many real-world networks vary over time, that is, the dataset can be represented as a sequence of graph snapshots. Hence, it is natural to consider the question of finding dense subgraphs in a temporal network that are allowed to vary over time to a certain degree. In this paper, we search for dense subgraphs that have large pairwise Jaccard similarity coefficients. More formally, given a set of graph snapshots and a weight $\lambda$, we find a collection of dense subgraphs such that the sum of densities of the induced subgraphs plus the sum of Jaccard indices, weighted by $\lambda$, is maximized. We prove that this problem is NP-hard. To discover dense subgraphs with good objective value, we present an iterative algorithm which runs in $\mathcal{O}(n^2k^2 + m \log n + k^3 n)$ time per single iteration, and a greedy algorithm which runs in $\mathcal{O}(n^2k^2 + m \log n + k^3 n)$ time, where $k$ is the length of the graph sequence and $n$ and $m$ denote number of nodes and total number of edges respectively. We show experimentally that our algorithms are efficient, they can find ground truth in synthetic datasets and provide interpretable results from real-world datasets. Finally, we present a case study that shows the usefulness of our problem.

==> stats-table-real.tex <==

\begin{table}[t!]
\setlength{\tabcolsep}{0pt}
\caption{
Computational statistics from the experiments with  real-world datasets. Here, $\lambda$ is used to handle the ratio between the terms in the objective if the algorithm is related to soft constraints otherwise it denotes the $\alpha$ value for the hard constraint algorithm, $i_1$ and $i_2$ give the number of iterations using Algorithm $\ref{alg:hard}$ and $\ref{alg:soft-1}$,
$d_{1}$, $d_2$ and $d_{3}$ are the discovered sum densities using Algorithm $\ref{alg:hard}$, $\ref{alg:soft-1}$, and  $\ref{alg:soft-2}$ respectively,  $o_2$ and $o_{3}$ are the discovered objective values for soft constrained algorithms,  $t_1$, $t_2$, and $t_3$ give the computational time in seconds, and  $j_{1}$ provides the  minimum pairwise Jaccard coefficient between discovered sets of vertices using Algorithm $\ref{alg:hard}$. 
}

\label{tab:stats3}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {dataset,l_alpha,dis_d_0,dis_d_1,dis_d_2,dis_obj_1,dis_obj_2,time_0,time_1,time_2,itr_0,itr_1,min_jac_dis_0},
    columns/dataset/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Data}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{V}$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E}$},
    columns/tau/.style={fixed, set thousands separator={\,}, column type=r, column name=$\tau$},
    columns/time_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$t_1$},
    columns/time_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$t_2$},
    columns/time_2/.style={fixed, set thousands separator={\,}, column type=r, column name=$t_3$},
    columns/l_alpha/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/true_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{true}$}, 
    columns/dcs_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$dcs$}, 
    columns/dense_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{l}$}, 
    columns/min_jac_dis_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{1}$}, 
    columns/min_jac_dis_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{2}$}, 
    columns/min_jac_dis_2/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{3}$}, 
    columns/avg_jac_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{1}$}, 
    columns/avg_jac_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{2}$}, 
    columns/avg_jac_2/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{3}$}, 
    columns/itr_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$i_1$},
    columns/itr_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$i_2$},
    columns/dis_d_0/.style={fixed,set thousands separator={\,}, column type=r, column name=$d_1$},
    columns/dis_d_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$d_2$},
    columns/dis_d_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$d_3$},
    columns/dis_obj_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$o_2$},
    columns/dis_obj_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$o_3$},
    every head row/.style={
		before row={
			\toprule
			\arraybackslash
			&      
      & \multicolumn{3}{l}{$den$} 
      & \multicolumn{2}{l}{$obj$} 
      &	\multicolumn{3}{l}{$time$}
      &  \multicolumn{2}{l}{$itr$}\\
                \cmidrule(lr){3-5}
			\cmidrule(lr){6-7}
			\cmidrule(lr){8-10}
			\cmidrule(lr){11-12}},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{real.csv}
\end{table}




==> stats-table-syn-com.tex <==

\begin{table}[t!]
\setlength{\tabcolsep}{0pt}
\caption{
Computational statistics from the experiments with the synthetic datasets. Here, $\lambda$ is used to handle the ratio between the terms in the objective if the algorithm is related to soft constraints otherwise it denotes the $\alpha$ value for the hard constraint algorithm, $i_1$ and $i_2$ give the number of iterations using Algorithm $\ref{alg:hard}$ and $\ref{alg:soft-1}$,
$d_{1}$, $d_2$, and $d_{3}$ are the discovered sum densities using Algorithm $\ref{alg:hard}$, $\ref{alg:soft-1}$, and  $\ref{alg:soft-2}$ respectively,  $o_2$ and $o_{3}$ are the discovered objective values for soft constrained algorithms, $j_{1}$, $j_{2}$, and $j_{3}$ provide the  minimum pairwise Jaccard coefficients between discovered sets of vertices, $a_{1}$, $a_{2}$, and $a_{3}$ give the  average pairwise Jaccard coefficients between discovered and ground-truth sets of vertices,  and    $t_1$, $t_2$, and $t_3$ give the computational time in seconds.
}

\label{tab:stats2}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {dataset,l_alpha,itr_0,itr_1,dis_d_0,dis_d_1,dis_d_2,dis_obj_1,dis_obj_2,min_jac_dis_0,min_jac_dis_1,min_jac_dis_2,avg_jac_0,avg_jac_1,avg_jac_2,time_0,time_1,time_2},
    columns/dataset/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Data}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{V}$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$Exp[\abs{E}]$},
    columns/time_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$t_1$},
    columns/time_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$t_2$},
    columns/time_2/.style={fixed, set thousands separator={\,}, column type=r, column name=$t_3$},
    columns/l_alpha/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/true_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{true}$}, 
    columns/dcs_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{dcs}$}, 
    columns/dense_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{den}$}, 
    columns/min_jac_dis_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{1}$}, 
    columns/min_jac_dis_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{2}$}, 
    columns/min_jac_dis_2/.style={fixed, set thousands separator={\,}, column type=r, column name=$j_{3}$}, 
    columns/avg_jac_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$a_{1}$}, 
    columns/avg_jac_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$a_{2}$}, 
    columns/avg_jac_2/.style={fixed, set thousands separator={\,}, column type=r, column name=$a_{3}$}, 
    columns/itr_0/.style={fixed, set thousands separator={\,}, column type=r, column name=$i_1$},
    columns/itr_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$i_2$},
    columns/dis_d_0/.style={fixed,set thousands separator={\,}, column type=r, column name=$d_1$},
    columns/dis_d_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$d_2$},
    columns/dis_d_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$d_3$},
    columns/dis_obj_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$o_2$},
    columns/dis_obj_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$o_3$},
    every head row/.style={
		before row={
			\toprule
			\arraybackslash
			& & 
      \multicolumn{2}{l}{$itr$}
      & \multicolumn{3}{l}{$den_{dis}$} 
      & \multicolumn{2}{l}{$obj_{dis}$} 
      &   \multicolumn{3}{l}{$J_{min}$}
      &	\multicolumn{3}{l}{$J_{avg}$}
      &	\multicolumn{3}{l}{$time$} \\
                \cmidrule(lr){3-4}
			\cmidrule(lr){5-7}
			\cmidrule(lr){8-9}
			\cmidrule(lr){10-12}
                \cmidrule(lr){13-15}
			\cmidrule(lr){16-18}},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{c2.csv}
\end{table}




==> statstable-2.tex <==

\begin{table}[t!]
\setlength{\tabcolsep}{0pt}
\caption{Statistics from the experiments with the synthetic datasets. Here, $\tau$  is the number of snapshots, $\lambda$ is used to handle the ratio of the terms in the objective, $d_{true}$ and $d_{dis}$ are the ground truth and discovered sum densities respectively, $J_{min}$ minimum pairwise Jaccard coefficients between discovered sets of vertices, and $time$ gives the computational time in seconds for Algorithm~$\ref{alg:soft-2}$.
}

\label{tab:stats21}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,n,m,tau,lam,grd_den,dis_den,min_jac,time},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{V}$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E}$},
    columns/tau/.style={fixed, set thousands separator={\,}, column type=r, column name=$\tau$},
    columns/lam/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/grd_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{true}$}, 
    columns/dis_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{dis}$}, 
    columns/min_jac/.style={fixed, set thousands separator={\,}, column type=r, column name=$J_{min}$}, 
    columns/itr/.style={fixed, set thousands separator={\,}, column type=r, column name=$itr$},
    columns/time/.style={fixed,set thousands separator={\,}, column type=r, column name=$time$},
    every head row/.style={
		before row={\toprule},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{table-2.csv}
\end{table}




==> statstable-com.tex <==

\begin{table}[t!]
\setlength{\tabcolsep}{0pt}
\caption{Statistics from the experiments with the synthetic datasets. Here, $\tau$  is the number of snapshots, $\lambda$ is used to handle the ratio of the terms in the objective, $d_{true}$ and $d_{dis}$ are the ground truth and discovered sum densities respectively, $J_{min}$ minimum pairwise Jaccard coefficients between discovered sets of vertices, $itr$ gives the number of iterations using Algorithm $\ref{alg:soft-1}$ , and $time$ gives the computational time in seconds for Algorithm $\ref{alg:soft-1}$.
}

\label{tab:stats2}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,n,m,tau,lam,grd_den,dis_den,min_jac,itr,time},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{V}$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E}$},
    columns/tau/.style={fixed, set thousands separator={\,}, column type=r, column name=$\tau$},
    columns/lam/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/grd_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{true}$}, 
    columns/dis_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{dis}$}, 
    columns/min_jac/.style={fixed, set thousands separator={\,}, column type=r, column name=$J_{min}$}, 
    columns/itr/.style={fixed, set thousands separator={\,}, column type=r, column name=$itr$},
    columns/time/.style={fixed,set thousands separator={\,}, column type=r, column name=$time$},
    every head row/.style={
		before row={\toprule},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{table-1.csv}
\end{table}




==> statstable-multi-row.tex <==

\begin{table*}[t]
\caption{Sizes and computational times for the synthetic and real-world datasets. 
}
\label{tab:stats-multi}

\pgfplotstabletypeset[
    begin table={\begin{tabular*}{1.2\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name,n,m,tau,true_den,dcs_den,min_jac_gnd,alpha,l,dis_d_0,dis_d_1,dis_d_2,dis_obj_0,dis_obj_1,dis_obj_2,avg_jac_0,avg_jac_1,avg_jac_2,time_0,time_1,time_2,itr},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{V}$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$\abs{E}$},
    columns/tau/.style={fixed, set thousands separator={\,}, column type=r, column name=$\tau$},
    columns/true_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{true}$}, 
    columns/dcs_den/.style={fixed, set thousands separator={\,}, column type=r, column name=$d_{dcs}$}, 
    columns/alpha/.style={fixed, set thousands separator={\,}, column type=r, column name=$\alpha$},
    columns/l/.style={fixed, set thousands separator={\,}, column type=r, column name=$\lambda$},
    columns/min_jac_gnd/.style={fixed, set thousands separator={\,}, column type=r, column name=$J_{min}$}, 
    columns/dis_d_0/.style={fixed,set thousands separator={\,}, column type=r, column name=$\alghard$},
    columns/dis_d_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsoftone$},
    columns/dis_d_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsofttwo$},
    columns/dis_obj_0/.style={fixed,set thousands separator={\,}, column type=r, column name=$\alghard$},
    columns/dis_obj_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsoftone$},
    columns/dis_obj_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsofttwo$},
    columns/avg_jac_0/.style={fixed,set thousands separator={\,}, column type=r, column name=$\alghard$},
    columns/avg_jac_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsoftone$},
    columns/avg_jac_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsofttwo$},
    columns/time_0/.style={fixed,set thousands separator={\,}, column type=r, column name=$\alghard$},
    columns/time_1/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsoftone$},
    columns/time_2/.style={fixed,set thousands separator={\,}, column type=r, column name=$\algsofttwo$},
    columns/itr/.style={fixed, set thousands separator={\,}, column type=r, column name=itr},
    every head row/.style={
		before row={
			\toprule
			\arraybackslash
			& & & & & & & & & \multicolumn{3}{l}{$d_{dis}$} & \multicolumn{3}{l}{$d_{dis}$} &
		    \multicolumn{3}{l}{$Jac_{avg}$} &	\multicolumn{3}{l}{$time(s)$} \\
			\cmidrule(lr){10-12}
			\cmidrule(lr){13-15}
			\cmidrule(lr){16-18}
			\cmidrule(lr){19-21}},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{stats-multi-row.csv}
\end{table*}


==> statstable-real.tex <==
\begin{table}[t]
\caption{Sizes and computational times for the real-time datasets. Here, $n$ is
the number of nodes, $m$ is the number of edges, $R$ is the number of groups, $K$ is the number of segments, $H$ is the number of levels, $LL$ is the  normalized log-likelihood, $I$ is the number of iterations, and $CT$ is the computational time in seconds.
}
\label{tab:stats2}
\setlength{\tabcolsep}{0pt}


\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name, n, m,  L, K, H,LL_1, I, R},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$n$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$m$},
    columns/L/.style={fixed, set thousands separator={\,}, column type=r, column name=$R$},
    columns/K/.style={fixed, set thousands separator={\,}, column type=r, column name=$K$},
    columns/H/.style={fixed, set thousands separator={\,}, column type=r, column name=$H$},
    columns/LL_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$LL$},
    columns/I/.style={fixed, set thousands separator={\,}, column type=r, column name=$I$},
    columns/R/.style={string type, column type=r, column name=$CT$},
    every head row/.style={
		before row={\toprule},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{st2.csv}
\end{table}


==> statstable-synthetic.tex <==

\begin{table}[t!]
\setlength{\tabcolsep}{0pt}
\caption{Experiments for the synthetic datasets. Here, $n$ is
the number of nodes, $m$ is the number of edges, $R$ is the number of groups, $K$ is the number of segments, $H$ is the number of levels, $LL_1$ is the normalized log-likelihood for the ground truth, $G$ is the Rand index, $LL_2$ is the discovered normalized log-likelihood, $I$ is
the number of iterations, and $CT$ is the computational time in seconds. }

\label{tab:stats1}
\pgfplotstabletypeset[
    begin table={\begin{tabular*}{\textwidth}},
    end table={\end{tabular*}},
    col sep=comma,
	columns = {name, n, m, L, K, H,LL_1, R,LL_2,I,CT},
    columns/name/.style={string type, column type={@{\extracolsep{\fill}}l}, column name=\emph{Dataset}},
    columns/n/.style={fixed, set thousands separator={\,}, column type=r, column name=$n$},
    columns/m/.style={fixed, set thousands separator={\,}, column type=r, column name=$m$},
    columns/L/.style={fixed, set thousands separator={\,}, column type=r, column name=$R$},
    columns/K/.style={fixed, set thousands separator={\,}, column type=r, column name=$K$},
    columns/H/.style={fixed, set thousands separator={\,}, column type=r, column name=$H$},
    columns/LL_1/.style={fixed, set thousands separator={\,}, column type=r, column name=$LL_1$},
    columns/R/.style={fixed, set thousands separator={\,}, column type=r, column name=$G$},
    columns/LL_2/.style={fixed, set thousands separator={\,}, column type=r, column name=$LL_2$},
    columns/I/.style={fixed, set thousands separator={\,}, column type=r, column name=$I$},
    columns/CT/.style={string type, column type=r, column name=$CT$},
    every head row/.style={
		before row={\toprule},
			after row=\midrule},
    every last row/.style={after row=\bottomrule},
]
{st1.csv}
\end{table}




==> synthetic-sample.tex <==
\begin{figure}[ht!]
\setlength{\tabcolsep}{2pt}
\newlength{\synfigheight}
\setlength{\synfigheight}{3.3cm}
\newlength{\synfigwidth}
\setlength{\synfigwidth}{4.5cm}
\begin{tabular}{ll}
\begin{tikzpicture}
\begin{axis}[xlabel={time}, ylabel= {$\lambda_{\mathrm{11}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.3,
    ymax = 0.6,
    scaled y ticks = false,
    cycle list name=yaf,
    % label style={font=\scriptsize},
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y1, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.3}{.6}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={time}, ylabel= {  $\abs{\lambda_{\mathrm{11}}(t) - \lambda'_{\mathrm{11}}(t)}$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.0,
    ymax = 0.002,
    scaled y ticks = true,
    cycle list name=yaf,
    % label style={font=\scriptsize},
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y1-y2, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{0.0}{.002}}
\end{axis}
\end{tikzpicture}\\

\begin{tikzpicture}
\begin{axis}[xlabel={time}, ylabel= { $\lambda_{\mathrm{12}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.0,
    ymax = 0.6,
    scaled y ticks = false,
    cycle list name=yaf,
    % label style={font=\scriptsize},
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y3, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.0}{.6}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={time}, ylabel= { $\abs{\lambda_{\mathrm{12}}(t) - \lambda'_{\mathrm{12}}(t)}$ },
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.0,
    ymax = 0.0004,
    scaled y ticks = true,
    cycle list name=yaf,
    % label style={font=\scriptsize},
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y3-y4, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.0}{.0004}}
\end{axis}
\end{tikzpicture}\\

\iffalse
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {true $\lambda_{\mathrm{13}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.3,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    label style={font=\scriptsize},
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y5, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.3}{.7}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {estimated $\lambda_{\mathrm{13}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.3,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y6, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.3}{.7}}
\end{axis}
\end{tikzpicture}\\

\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {true $\lambda_{\mathrm{22}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.05,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y7, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.05}{.7}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {estimated $\lambda_{\mathrm{22}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.05,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y8, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.05}{.7}}
\end{axis}
\end{tikzpicture}\\
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {true $\lambda_{\mathrm{23}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.1,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y9, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.1}{.7}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {estimated $\lambda_{\mathrm{23}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.1,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y10, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.1}{.7}}
\end{axis}
\end{tikzpicture}\\

\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {true $\lambda_{\mathrm{33}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.17,
    ymax = 0.28,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y11, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.17}{.28}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {estimated $\lambda_{\mathrm{33}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.17,
    ymax = 0.28,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y12, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.17}{.28}}
\end{axis}
\end{tikzpicture}
\fi


\end{tabular}
\caption{True parameters $\lambda_{\mathrm{11}}(t)$, $\lambda_{\mathrm{12}}(t)$ (left) and their difference to the estimated estimated parameters $\lambda'_{\mathrm{11}}(t)$, $\lambda'_{\mathrm{12}}(t)$(right) for the
\dtname{Synthetic-4} dataset. $\lambda_{\mathrm{12}}(t)$ implies the Poisson process parameter between group $1$ and group $2$ as a function of time. This experiment is done with $n=60$,
$m=537\,501$, $R=3$, $K=4$, and $H=3$. 
}
\label{fig:intensity-2}
\end{figure}


==> synthetic.tex <==
\begin{figure}[ht!]
\setlength{\tabcolsep}{0pt}
\newlength{\synfigheight}
\setlength{\synfigheight}{3.4cm}
\newlength{\synfigwidth}
\setlength{\synfigwidth}{4.5cm}
\begin{tabular}{ll}
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Generated $\lambda_{\mathrm{11}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.3,
    ymax = 0.6,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y1, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.3}{.6}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Discovered $\lambda_{\mathrm{11}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.3,
    ymax = 0.6,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y2, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.3}{.6}}
\end{axis}
\end{tikzpicture}\\

\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Generated $\lambda_{\mathrm{12}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.075,
    ymax = 0.6,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y3, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.075}{.6}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Discovered $\lambda_{\mathrm{12}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.075,
    ymax = 0.6,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y4, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.075}{.6}}
\end{axis}
\end{tikzpicture}\\

\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Generated $\lambda_{\mathrm{13}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.3,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y5, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.3}{.7}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Discovered $\lambda_{\mathrm{13}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.3,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y6, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.3}{.7}}
\end{axis}
\end{tikzpicture}\\

\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Generated $\lambda_{\mathrm{22}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.05,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y7, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.05}{.7}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Discovered $\lambda_{\mathrm{22}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.05,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y8, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.05}{.7}}
\end{axis}
\end{tikzpicture}\\
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Generated $\lambda_{\mathrm{23}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.1,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y9, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.1}{.7}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Discovered $\lambda_{\mathrm{23}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.1,
    ymax = 0.7,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y10, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.1}{.7}}
\end{axis}
\end{tikzpicture}\\

\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Generated $\lambda_{\mathrm{33}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.17,
    ymax = 0.28,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y11, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.17}{.28}}
\end{axis}
\end{tikzpicture}&
\begin{tikzpicture}
\begin{axis}[xlabel={$t$}, ylabel= {Discovered $\lambda_{\mathrm{33}}(t)$},
    width = \synfigwidth,
    height = \synfigheight,
    xmin = 0,
    xmax = 800,
    ymin = 0.17,
    ymax = 0.28,
    scaled y ticks = false,
    cycle list name=yaf,
    yticklabel style={/pgf/number format/fixed},
    no markers,
]
\addplot table [x=x, y=y12, col sep=comma] {lamb-2.csv};
\pgfplotsextra{\yafdrawaxis{0}{800}{.17}{.28}}
\end{axis}
\end{tikzpicture}


\end{tabular}
\caption{Generated (left) vs discovered (right) intensity functions
($\lambda_{\mathrm{11}}(t)$, $\lambda_{\mathrm{12}}(t)$,
$\lambda_{\mathrm{13}}(t)$, $\lambda_{\mathrm{22}}(t)$,
$\lambda_{\mathrm{23}}(t)$, and $\lambda_{\mathrm{33}}(t)$) for the
\dtname{Synthetic-4} dataset. $\lambda_{\mathrm{12}}(t)$ implies the intensity
function between group $1$ and group $2$. This experiment is done with $n=60$,
$m=537\,501$, $R=3$, $K=4$, and $H=3$. 
}
\label{fig:intensity-2}
\end{figure}

